iJTyper: An Iterative Type Inference Framework for Java by Integrating Constraint- and Statistically-based Methods

Inferring the types of API elements in incomplete code snippets (e.g., those on Q&A forums) is a prepositive step required to work with the code snippets. Existing type inference methods can be mainly categorized as constraint-based or statistically-based. The former imposes higher requirements on code syntax and often suffers from low recall due to the syntactic limitation of code snippets. The latter relies on the statistical regularities learned from a training corpus and does not take full advantage of the type constraints in code snippets, which may lead to low precision. In this paper, we propose an iterative type inference framework for Java, called iJTyper, by integrating the strengths of both constraint- and statistically-based methods. For a code snippet, iJTyper first applies a constraint-based method and augments the code context with the inferred types of API elements. iJTyper then applies a statistically-based method to the augmented code snippet. The predicted candidate types of API elements are further used to improve the constraint-based method by reducing its pre-built knowledge base. iJTyper iteratively executes both methods and performs code context augmentation and knowledge base reduction until a termination condition is satisfied. Finally, the final inference results are obtained by combining the results of both methods. We evaluated iJTyper on two open-source datasets. Results show that 1) iJTyper achieves high average precision/recall of 97.31% and 92.52% on both datasets; 2) iJTyper significantly improves the recall of two state-of-the-art baselines, SnR and MLMTyper, by at least 7.31% and 27.44%, respectively; and 3) iJTyper improves the average precision/recall of the popular language model, ChatGPT, by 3.25% and 0.51% on both datasets.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf

BIBLATEXFILES= $(wildcard *.bbx) $(wildcard *.cbx) $(wildcard *.dbx) $(wildcard *.lbx)
SAMPLEBIBLATEXFILES=$(patsubst %,samples/%,$(BIBLATEXFILES))

all:  ${PDF} ALLSAMPLES

%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES: $(SAMPLEBIBLATEXFILES)
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/abbrev.bib: ACM-Reference-Format.bst
	perl -pe 's/MACRO ({[^}]*}) *\n/MACRO \1/' ACM-Reference-Format.bst \
	| grep MACRO | sed 's/MACRO {/@STRING{/' \
	| sed 's/}  *{/ = /' > samples/abbrev.bib 


samples/%.bbx: %.bbx
samples/%.cbx: %.cbx
samples/%.dbx: %.dbx
samples/%.lbx: %.lbx

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-sigconf-biblatex.pdf: samples/sample-sigconf-biblatex.tex $(SAMPLEBIBLATEXFILES)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && biber $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-acmsmall-biblatex.pdf: samples/sample-acmsmall-biblatex.tex $(SAMPLEBIBLATEXFILES)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && biber $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex-dev $(notdir $<)
	cd $(dir $@) && xelatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex-dev $(notdir $<); done

samples/sample-lualatex.pdf:  samples/sample-lualatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex-dev $(notdir $<)
	cd $(dir $@) && lualatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex-dev $(notdir $<); done

samples/sample-acmcp.pdf: samples/acm-jdslogo.png

.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut \
	samples/acm-jdslogo.png \
	samples/*.run.xml samples/*.bcf $(SAMPLEBIBLATEXFILES)


clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

# distros
distros: all docclean
	zip -r acm-distro.zip  \
	acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.* \
	--exclude samples/sample-acmengage*
	zip -r acmengage-distro.zip samples/sample-acmengage* \
	samples/*.bib \
	acmart.pdf acmguide.pdf  *.cls ACM-Reference-Format.*


.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

Version 1.90   Journal ISSN updated

Version 1.89a  Added version info to .bst

Version 1.89   Bug fixes
	       Redesign of ACMCP
	       New positioning of badges
	       New journals: PACMMOD, TOPML

Version 1.88   New ISSNs
	       Documentation updates
	       New journal:  PACMNET

Version 1.87   CC license is allowed for non-acm documents and ACM Engage
	       documents only
	       New format acmcp for the cover page
	       New journals: JATS, ACMJCSS, TORS
	       Bug fixes

Version 1.86.  Empty country in affiliation now produces an error
               Bug fixes
	       New samples for acmengage

Version 1.85.  Bug fixes
	       Added support for Creative Commons licenses (requires
	       doclicense images)
	       New journals
	       New format acmengage for ACM Engage CSEdu course materials 

Version 1.84   Support for BibLaTeX rewritten (thanks to
	       Roberto Di Cosmo and Kartik Singhal)
	       Corrected German translation (thanks to Dirk Beyer)
	       New journals

Version 1.83   Support for multilanguage papers
	       ISSN changes for some journals

Version 1.82   Bug fixes.
	       New command \anon for anonymization of short strings.
	       Documentation update.

Version 1.81   Bug fixes
	       New bib field distinctURL to print URL even if doi is present.
	       Reworded samples

Version 1.80   New journals: DLT, FAC

Version 1.79   Fixed pages with index
	       (https://github.com/borisveytsman/acmart/issues/440)
	       Updated information for TAP, TCPS, TEAC

Version 1.78   Documentation update.
	       Magic texcount comments for samples.
	       Title page now is split if there are too many authors
	       Bug fixes.

Version 1.77   Changed the way to typeset multiple affiliations (Christoph Sommer)

Version 1.76   Added many journal abbreviations to the bst.
	       New experimental option: pbalance
	       ORCID linking code

Version 1.75   Omitted \country now produces error.
	       Added \AtBeginMaketitle

Version 1.74   Bug fixes.  A regression introduced in the font changes
	       is reverted.

Version 1.73   Bug fixes
	       The elements institution, city and country are now obligatory
	       for affiliations.  The absence of them produces a warning

Version 1.72   Bug fixes.  Better handling of metadata.

Version 1.71   Bug fixes
               Formats sigchi and sigchi-a are retired
	       Bibliography formatting changes for @inproceedings entries
	       having both series and volume
	       LuaLaTeX now uses the same OTF fonts as XeLaTeX

Version 1.70   Title change for ACM/IMS Transactions on Data Science
               Bug fixes for bibliography

Version 1.69   Bug fixes
	       Compatibility with LaTeX 2020-02-02 release

Version 1.68   Bug fixes
               BST now recognizes words `Paper' or 'Article' in
	       eid or articleno

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.63a   Moved TQUANT to TQC

Version 1.63	New journals: TQUANT, FACMP

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.52    Another rewording of licenses

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.49    New jorunal:  DTRAP

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.47    New journal: THRI

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.43    Bug fixes

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.41    Rearranged bib files
                Added new badges

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.39    Added \authornotemark commmand

Version 1.38    Increase default font size for SIGPLAN

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

Version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

Version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

Version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

Version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

Version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

Version 1.28    Bug fixes: natbib=false now behaves correctly.

Version 1.27    Bug fixes

Version 1.26    Bug fixes

Version 1.25    Updated PACMPL journal option.

Version 1.24    Added IMWUT journal option.

Version 1.23    Added PACM PL journal option.

Version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

Version 1.21    Bibliography changes: added arXiv, some cleanup

Version 1.20    Bug fixes, documentation updates

Version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

Version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.


Version 1.17    Formatting changes for margins and lists.  Bug fixes.

Version 1.16    Formatting changes for headers and footers.

Version 1.15    New structured affiliation command.
                New commands for acknowledgements.

Version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

Version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

Version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

Version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

Version 1.10    Bug fixes

Version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

Version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes


==> methodology-1.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{figure/fig4_framework.pdf}
    \caption{The framework of \MethodName.}
    \label{fig:overview}
\end{figure}

Fig.~\ref{fig:overview} shows an overview framework of our proposed \MethodName{}. The input is a code snippet, and the output is the code snippet with inferred types of the API elements (primarily the classes and interfaces) in it. \MethodName{} contains four main steps \circled{1}-\circled{4}. At first, \MethodName{} applies a constraint-based type inference method, e.g., SnR~\cite{DBLP:conf/icse/DongGTS22}, to the code snippet (\circled{1}). Since the inference results may contain missing or wrong types due to the limitations of the method (as explained in Section~\ref{subsec:ctim}), which could be partially addressed using statistically-based methods, \MethodName{} further feed the code snippet augmented with the inferred types to a statistically-based type inference method, e.g., MLMTyper~\cite{DBLP:conf/kbse/HuangYXX0022-prompt} (\circled{2}). In turn, the top-$k$ candidate types predicted by method could be used to improve the constraint-based method by filtering irrelevant types in the pre-built KB. Therefore, \MethodName{} adopts an iterative mechanism. After performing a round of both methods, \MethodName{} examines whether some termination conditions (e.g., the inference results become stable or a maximum number of iterations is reached) are satisfied. If the examination answer is negative, \MethodName{} reduces the KB of the constraint-based method using the top-$k$ candidate types of each API element predicted by the statistically-based method (\circled{3}) and then re-applies the constraint-based method to the code snippet. After the iteration is terminated, \MethodName{} combines the inference results of both methods to produce the final inference results (\circled{4}).

Please notice that \MethodName{} is a flexible framework which can integrate different constraint-based and statistically-based methods. In this work, we demonstrate the framework using two state-of-the-art methods, i.e., SnR and MLMTyper, for instance. In addtion, based on our literature review, we find that some constraint-based methods are complex and their replication packages are also difficult to understand and modify. For example, the implementation code in the replication package\footnote{\url{https://doi.org/10.5281/zenodo.5843327}} of SnR is obfuscated and compiled to a Jar file, making it hard to replicate and extend the work. In such cases, it requires great efforts to adjust the implementation to utilize the top-$k$ candidate types predicted by the statistically-based method. To save the efforts, we provide a simple solution (\circled{3}) to integrating any constraint-based method which has a workable replication package. Instead of adjusting the implementation code, \MethodName{} directly reduces the pre-built KB based on the top-$k$ candidate types. We acknowledge that this solution may sacrifice some efficiency, however it can help users escape from the efforts required to understand and modify the implementation of the constraint-based method and thus might be desired by users in non real-time application scenarios.

\subsection{Constraint-based Type Inference}

In this first step, for an input code snippet, we use a constraint-based type inference method to infer the types of the API elements. Due to the limitations of the method (see Section~\ref{subsec:ctim}), for some API elements, the inference may fail or the inferred types may be incorrect. For example, Fig.~\ref{fig:syntax-incorrectness} shows a code snippet with syntax errors, for which SnR fails to infer the types of four classes. Fig.~\ref{fig:context-augment} shows another code snippet from the SO post `3954392', which %which also contains five classes whose types need to be inferred, i.e., \{ \emph{ArrayList}[6,1], \emph{ArrayList}[6,2], \emph{Document}[7,1], \emph{Element}[9,1], \emph{DOM}[9,1] \}. Similar to Tables~\ref{tab:snr-syntax-incorrectness} and~\ref{fig:ase-disadvantage}, we label every specific API element with two indices, e.g., \emph{ArrayList}[6,1] refers to the first occurrence of \emph{ArrayList} at line 6. 
% Different from the example shown in Fig.~\ref{fig:syntax-incorrectness}, 
illustrates the limitation of SnR on the capability of extracting constraints from code snippets. By applying SnR to the code snippet, four classes get their right types, e.g., the type of \emph{Element}[9,1] is inferred as \emph{com.google.gwt.user.client.Element}, but there is no type inferred for \emph{Document}[7,1]. Through an in-depth analysis, we find that the class has nine candidate types in the pre-built KB. Although the KB contains the right type of the class, i.e., \emph{com.google.gwt.dom.client.Document}, SnR fails to determine the type. This issue is because SnR cannot effectively extract the full constraints expressed by the cascaded method calls, i.e., `\emph{Document.get().getBody()}', and thus cannot distinguish the right type from a noise type, i.e., \emph{com.extjs.gxt.ui.client.widget.Document}, which also has a method \emph{get()} but the return type does not have a method \emph{getBody()}.

As stated previously, the limitations of constraint-based methods can be partially addressed by statistically-based methods. This is because statistically-based methods have two main advantages: 1) They are not affected by the syntax errors in code snippets; and 2) They employ the context (e.g., the token co-occurrence) of API elements to predict the types without the need to extract constraints from code snippets. As presented in Table~\ref{tab:snr-syntax-incorrectness}, MLMTyper successfully predicts the right types for the four classes that fail to be inferred by SnR. Moreover, the types inferred by the constraint-based method could be used to augment the context of API elements in the code snippet and thus improve the performance of the statistically-based method. We build the augmented code snippet by replacing the API elements with their inferred types, which is formalized as follows.

\textbf{Context Augmentation of the Code Snippet.}
Recall that statistically-based methods treat the input code snippet as a plain text. Specifically, the code snippet can be denoted as a token sequence, $CS=t_{1}t_{2}...t_{m}$ where some of the tokens are API elements. The set of API elements, denoted as $APIs(CS)$, can be identified from the AST of $CS$ or using regular expressions if the AST generation is failed due to syntax errors. Based on the type inference results of the constraint-based method, $APIs(CS)$ can be divided into two subsets: the set of API elements with inferred types and the set of API elements without inferred types, which are denoted as $Typed\_APIs^{C}(CS)$ and $NonTyped\_APIs^{C}(CS)$, respectively. The inferred type of an API element $t_{i}\in Typed\_APIs^{C}(CS)$ is denoted as $type^{C}(t_{i})$. Then, the augmented code snippet can be represented as a new token sequence, $ACS=y_{1}y_{2}...y_{m}$ where the API elements are replaced with their types, i.e., 
\begin{equation}
    y_{i} = type^{C}(t_{i}) \text{ if } t_{i} \in Typed\_APIs^{C}(CS) \text{ else } t_{i}, \forall i = 1,...,m   
\end{equation}

\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{figure/fig5_context_augmentation.pdf}
    \caption{Example of the type inference results improved by leveraging the augmented code snippet using a code snippet from the SO post `3954392'. The types with a brown background are inferred by applying SnR to the original code snippet. The types in the yellow background box are predicted by MLMTyper before and after augmenting the original code snippet with the inferred types of SnR.}
    \label{fig:context-augment}
\end{figure}


\subsection{Statistically-based Type Inference}

In this step, a statistically-based type inference method, e.g., MLMTyper, is applied to the augmented code snippet $ACS$ built in the previous step. The common basis of statistically-based methods is the naturalness shared by most software, which is similar to that of natural language. Software naturalness~\cite{DBLP:journals/cacm/HindleBGS16-naturalness} means that human-written code is mostly simple, repetitive, and predictable, for which it can be modeled by statistical language models to assist developers with various software engineering tasks, such as type inference \cite{DBLP:conf/kbse/HuangYXX0022-prompt,DBLP:journals/scp/VelazquezRodriguezNR23-resico,DBLP:conf/icse/PhanNTTNN18-statype,DBLP:conf/kbse/SaifullahAR19-coster}, defect localization \cite{qiu2021deep-defect-localization,zhang2020softwareattention-defect-localization}, and code completion \cite{raychev2014statistical-codecompletion,svyatkovskiy2019pythia-code-completion}. Code context is used to capture such naturalness~\cite{DBLP:conf/kbse/SaifullahAR19-coster}, which is important for the performance of statistical models. The key difference between statistically-based type inference methods is the code context that they employ to predict the types of API elements. For example, STATTYPE~\cite{DBLP:conf/icse/PhanNTTNN18-statype} leverages type context and resolution context for type inference. The former refers to the classes, methods, and fields that occur around an API element, $e$, to be inferred, while the latter refers to the type inference decision of the API elements surrounding $e$. MLMTyper~\cite{DBLP:conf/kbse/HuangYXX0022-prompt} uses the code line where $e$ is located and the top and down $\eta$ (=2 by default) adjacent code lines to form a code context block.

We perform this step using the state-of-the-art statistically-based method, MLMTyper. MLMTyper has two execution modes which are called \emph{leave-one-out} and \emph{all-unknown} in~\cite{DBLP:conf/kbse/HuangYXX0022-prompt}. Specifically, during the execution of MLMTyper, it predicts each API element in the input code snippet one-by-one. For a specific API element, $e$, after building the code context block, the leave-one-out mode predicts the top-$k$ candidate types of $e$ with the known types of all the other API elements in the context. In contrast, the all-unknown mode predicts the types of $e$ without utilizing the types of any other API elements, i.e., assuming that those types are all unknown. The leave-one-out and all-unknown modes respectively represent the upper bound (i.e., the easiest case) and lower bound (i.e., the most difficult case) of type inference scenarios. We execute MLMTyper with the leave-one-out mode on the augmented code snippet $ACS$. However, it needs to point out that our execution is not strictly a leave-one-out mode because there can be some missing and/or incorrect types exist in $ACS$, as demonstrated in Figs.~\ref{fig:context-augment} and~\ref{fig:kb_reduction}. Considering the relatively high precision of {\color{blue}SnR} (see Table~\ref{tab:rq2-component}), the majority of the types in $ACS$ should be correct and thus can improve the performance of MLMTyper in most cases. Taking the code snippet shown in Fig.~\ref{fig:context-augment} as an example, before augmenting the code snippet, the top-1 type of the class \emph{Document}[7,1] predicted by MLMTyper, i.e., \emph{com.google.gwt.user.client.ui.Document}, is wrong, which is haphazardly generated by the language model and does not really exist. This problem is well-known as \emph{hallucination} \cite{ji2023survey-hallu,DBLP:conf/acl/ZhouNGDGZG21-hallu} of generative language models. After augmenting the code snippet with the inferred types of the other classes, MLMTyper successfully predicts the right type, i.e., \emph{com.google.gwt.dom.client.Document}, as the top-1 result. 

After this step, we obtain a list of candidate types predicted by MLMTyper for each API element in $ACS$ (or $CS$). Based on our observation, a considerable number of candidates are haphazardly generated, e.g., the wrong type shown in Fig.~\ref{fig:context-augment}. To solve this problem, we filter the candidates outside the pre-built KB of {\color{blue}SnR}. After that, the refined top-$k$ candidate types of an API element $e \in APIs(CS)$ are denoted as $types_{k}^{S}(e)$. These candidates are subsequently used to reduce the KB of SnR by filtering the types irrelevant to the API elements to improve the performance of SnR.

\begin{figure}%[ht]
    \centering
    \includegraphics[width=\linewidth]{figure/fig6_kb_reduction.pdf}
    \caption{Example of the type inference results improved by leveraging the reduced knowledge base (KB) using a code snippet from the SO post `39005622'. The types with a brown background are inferred by applying SnR to the original code snippet based on the pre-built KB. The types in the yellow background boxes are inferred by SnR before and after reducing the KB based on the top-$k$(=3) candidate types predicted by MLMTyper.}
    \label{fig:kb_reduction}
\end{figure}

\subsection{Knowledge Base Reduction}\label{chap:knowledge base reduction}

Constraint-based type inference methods search for the types of API elements in a code snippet from the pre-built KB. Generally, the KB should cover a large number of API libraries to ensure a good capability of the methods. As a result, there can be multiple candidate types of an API element in the KB. If the input code snippet does not contain sufficient constraints to determine the right type of an API element from the candidates, the methods will not be able to produce the desired answer. This limitation can be alleviated by leveraging the type inference results of statistically-based methods. Specifically, we introduce a KB reduction module in \MethodName{}.

The KB reduction module is proposed based on the assumption that the top-$k$ candidate types predicted by the statistically-based method for an API element $e$, i.e., $types_{k}^{S}(e)$, probably contain the right type of $e$. This assumption is supported by the evaluation results in~\cite{DBLP:conf/kbse/HuangYXX0022-prompt}, which reveal that the accuracy of the top-3 candidates is 91\% on a widely used dataset, StatType-SO \cite{DBLP:conf/icse/PhanNTTNN18-statype}. Therefore, the noise types of API elements in the pre-built KB of the constraint-based method can be reduced based on the top-$k$ candidates. Considering that the syntax knowledge of API elements is necessary for the constraint-based methods to solve the constraints extracted from code snippets, we implement the KB reduction module as two phases.

\textbf{Phase 1: Candidate Class \& Interface Type Collection.} In this first phase, we build a set of candidate types, denoted as $CanCITypes$, that can probably contain the right types of all classes and interfaces in the input code snippet. The reason why we focus on the classes and interfaces is explained in Section~\ref{subsec:titd}. At first, we collect the top-$k$ candidate types predicted for each class or interface, resulting in an initial $CanCITypes$. Since the performance of existing statistically-based methods is not perfect (e.g., the precision and recall of state-of-the-art MLMTyper are not 100\%), it is possible that the top-$k$ candidate types of a class or an interface do not contain the right type. Based on this consideration, if a class or an interface has a type inferred by the constraint-based method, and the type is not in $CanCITypes$, we add the type to $CanCITypes$ as it might be the right type. Finally, we formally define $CanCITypes$ as
\begin{equation}
    CanCITypes = \left(\bigcup_{e \in CIs(CS)} types_{k}^{S}(e)\right) \cup \left\{type^{C}(e)|e \in Typed\_APIs(CS) \cap CIs(CS)\right\}
\end{equation}
where $CIs(CS)$ represents the set of classes and interfaces in the input code snippet $CS$. It holds that $CIs(CS) \subseteq APIs(CS)$.

\textbf{Phase 2: Reduced KB Construction.} In this second phase, we construct a reduced KB by extracting the syntax knowledge of each class/interface type $ctype \in CanCITypes$ from the pre-built KB, denoted as $KB$, of the constraint-based method. The syntax knowledge includes the methods and fields declared in $ctype$, the super classes/interfaces of $ctype$ as well as their declared methods and fields. The reduced KB, denoted as $Reduced\_KB$, can be formally defined as
\begin{equation}
    Reduced\_KB = \bigcup_{ctype \in CanCITypes} Syn\_Knowl(ctype, KB)
\end{equation}
where $Syn\_Knowl(ctype, KB)$ represents the syntax knowledge of $ctype$ in $KB$.
\begin{equation}
    Syn\_Knowl(ctype, KB) = \bigcup_{e \in \{ctype \cup SupCITypes(ctype, KB)\}} e \cup e.Methods \cup e.Fields 
\end{equation}
where $SupCITypes(ctype, KB)$ represents the set of super class/interface types of $ctype$ in $KB$. For a class/interface type $e$, $e.Methods$ and $e.Fields$ are the set of methods and the set of fields declared in $e$, respectively. The reduced KB should also contain the relationships between the elements in it. 

\subsection{Iterative Type Inference} 
Based on the reduced KB, we can re-apply the constraint-based method to the input code snippet to obtain new inferred types of the API elements. Since many noise types are excluded in the reduced KB, the quality of the inferred types could be improved. Fig.~\ref{fig:kb_reduction} shows an example code snippet from the SO post `39005622'. Before reducing the pre-built KB, the types inferred by SnR for the interface \emph{Converter}[1,1] and the class \emph{UnmarshallingContext}[16,1] are both wrong. %, i.e., \emph{com.sun.xml.internal.ws.commons.xmlutil.Converter} and \emph{com.sun.xml.internal.bind.v2.runtime.unmarshaller.UnmarshallingContext}, are both wrong. 
After reducing the KB, SnR infers the right types for them because the two wrong types are excluded in the reduced KB. The right type of the class \emph{Document}[7,1] shown in Fig.~\ref{fig:context-augment} is also successfully inferred by SnR based on the reduced KB. These cases demonstrate the benefit of our KB reduction strategy.

Furthermore, it should be reasonable to assume that the new set of types with higher quality inferred by the constraint-based method can be used to better augment the code snippet and thus improve the performance of statistically-based method again. Considering this \textbf{mutual promotion effect} between the two methods, \MethodName{} adopts an iterative mechanism, as shown in Fig.~\ref{fig:overview}. Some termination conditions need to be set to control the iteration. Currently, we set two conditions: 1) The inference results are stable or 2) The number of iterations exceeds a threshold $\delta$ (=10 in this work). The second condition is used to avoid infinite iteration due to repeated oscillations in the results. After performing a round of both methods, \MethodName{} examines the two termination conditions. For condition 1), it compares the newly inferred types of both methods with those produced in the previous round. If they are the same, the inference results become stable. For condition 2), it compares the executed number of rounds, e.g., $rnum$, with $\delta$ to see whether $rnum$ is equal to $\delta$. The iteration ends when either of the two conditions is satisfied.

\subsection{Type Inference Result Combination}
After the iterative type inference process is terminated, we combine the inference results of the constraint-based method and the statistically-based method to produce the final inference results of \MethodName{}. The combination is performed in two phases.

\textbf{Phase 1: Combining the Inference Results of Each Method.} Through our observation from the experiments, there can be fluctuations exist in the results produced by either of the two methods during the iteration process. One case is that the type(s) of an API element inferred by a method in one round may differ from those in another round. Another case is that the inference of an API element by a method may fail in one round but succeed in another round. Moreover, {\color{blue}the results obtained by a method in a specific round (e.g., the last round) may not be the best, which is verified in the experiments of RQ1.} Unfortunately, in practical application of \MethodName{}, there is no way to design the optimal combination stategy which can find the maximum number of right types inferred for the API elements from the results produced in different rounds, without knowing the ground truth. We combine the inference results of each method using a simple strategy, i.e., keeping the last successfully inferred type(s) of each API element. After this phase, we denote the type of an API element, $e$, inferred by the constraint-based method as $comb\_type^{C}(e)$ and the top-$k$ candidate types of $e$ predicted by the statistically-based method as $comb\_types_{k}^{S}(e)$.

\textbf{Phase 2: Combining the Inference Results of Both Methods.} In this phase, we combine the combined results of both methods. Since the precision of constraint-based methods, e.g., SnR, is generally higher than that of statistically-based methods, e.g., MLMTyper\footnote{The evaluation results in~\cite{DBLP:conf/kbse/HuangYXX0022-prompt} show that MLMTyper achieves higher average accuracy than SnR on the StatType-SO dataset. However, the accuracy of MLMTyper is measured on the top-3 candidate types of each API element. According to our replication experiments, the average accuracy of the top-1 type predicted by MLMTyper is 66.89\%, which is much lower than that of SnR, i.e., 96.36\%, as presented in Table~\ref{tab:rq2-component}.}, we combine the type(s) of an API element, $e$, inferred by both methods according to two criteria: 1) If only the statistically-based method predicts the top-$k$ candidate types of $e$, i.e., $comb\_type^{C}(e) = null \wedge comb\_types_{k}^{S}(e) \neq \emptyset$, then the top-1 type, i.e., $comb\_types_{1}^{S}(e)$, is determined as the final type of $e$; 2) If both methods produce types for $e$, i.e., $comb\_type^{C}(e) \neq null \wedge comb\_types_{k}^{S}(e) \neq \emptyset$, then the type inferred by the constraint-based method, i.e., $comb\_type^{C}(e)$, is accepted as the final type of $e$.


==> motivation-1.tex <==
\subsection{Type Inference Task Description}\label{subsec:titd}
  
\begin{figure}%[htbp]
    \centering
    \includegraphics[width=0.8\linewidth]{figure/fig1_problem_description.pdf}
    \caption{Example code snippet annotated with four kinds of API elements from the SO post `442496'.}
    \label{fig:problem-description}
\end{figure}

Type reference task aims to identify the concrete types (i.e., fully qualified names (FQNs)) of API elements in an incomplete program, e.g., a code snippet. In general, there are five kinds of API elements whose types need to be inferred, i.e., \emph{classes}, \emph{interfaces}, \emph{methods}, \emph{fields}, and \emph{variables}.
Fig.~\ref{fig:problem-description} shows an example code snippet from the question post `442496' at Stack Overflow (SO). The classes, methods, fields, and variables are marked with yellow, blue, grey, and pink backgrounds, respectively. 

Among the API elements, classes and interfaces are more important since the types of classes and interfaces, together with the syntax knowledge (e.g., the declared methods and fields and the inheritance and implementation relationships) of them, can be used to infer the types of the other elements. For example, for the code snippet shown in Fig.~\ref{fig:problem-description}, after determining the type of the class `\emph{Inet4Address}' as `\emph{java.net.Inet4Address}', the type of the method `\emph{getByName("thehost")}' invoked by the class can be inferred as `\emph{public static InetAddress getByName(String host) throws UnknownHostException}' by leveraging the syntax knowledge of the class\footnote{https://docs.oracle.com/en/java/javase/17/docs/api/java.base/java/net/Inet4Address.html}. The type of the variable \emph{server} can be further inferred based on the return type of the method. Based on this insight, existing type inference methods primarily focus on identifying the types of classes and interfaces. Moreover, the classes that correspond to primitive data types, e.g., \emph{int} and \emph{Integer}, are often excluded because such types are easy to recognize and thus inferring them is meaningless. \textbf{Similarly, in this work, we focus on the type inference of classes and interfaces except those corresponding to primitive data types when describing our proposed \MethodName{} framework.}

\subsection{Limitations of Type Inference Methods}\label{sec:mlim}

Existing type inference methods proposed for Java programs can be categorized as two groups: constraint-based~\cite{DBLP:conf/icse/SubramanianIH14-baker,DBLP:conf/kbse/Shokri21-ase_depres,DBLP:conf/icse/DongGTS22} and statistically-based~\cite{DBLP:conf/icse/PhanNTTNN18-statype,DBLP:conf/kbse/SaifullahAR19-coster,DBLP:journals/scp/VelazquezRodriguezNR23-resico,DBLP:conf/kbse/HuangYXX0022-prompt}.

\begin{table}
    \centering
    \caption{Constraint-based type inference methods.}
    \label{tab:constraint-methods-review}
    \resizebox{\textwidth}{!}
    {
        \begin{tabular}{l|c|l} 
            \hline
            \multicolumn{1}{c|}{\textbf{Method}} & \textbf{Publication} & \multicolumn{1}{c}{\textbf{Summary}}                                                                                                                                                                                     \\ 
            \hline
            Baker~\cite{DBLP:conf/icse/SubramanianIH14-baker}                                & ICSE 2014            & \begin{tabular}[c]{@{}l@{}}Baker maintains a candidate list for each API and applies heuristic~rules to reduce the\\number of candidates deductively.\end{tabular}                                                       \\ 
            \hline
            DepRes~\cite{DBLP:conf/kbse/Shokri21-ase_depres}                               & ASE 2021             & \begin{tabular}[c]{@{}l@{}}DepRes generates a sketch for each API and utilizes a Z3 SMT~Solver to handle the \\constraints, aiming to find a minimum number~of types and dependencies.\end{tabular}                      \\ 
            \hline
            SnR~\cite{DBLP:conf/icse/DongGTS22}                                  & ICSE 2022            & \begin{tabular}[c]{@{}l@{}}SnR builds a knowledge base for generics and utilizes Datalog~to solve the~constraints. \\It ranks the candidates based on a~prioritization heuristic and selects the top item.\end{tabular}  \\ 
            \hline
            \multicolumn{1}{l}{}                 & \multicolumn{1}{l}{} &                                                                                                                                                                                                                         
            \end{tabular}
    }
\end{table}

\subsubsection{Constraint-based Type Inference Methods.}\label{subsec:ctim} Typically, a constraint-based method pre-builds a knowledge base (KB) that stores the syntax knowledge of API elements from a set of API libraries. Then, given a code snippet, it extracts type constraints between the API elements hidden in the code snippet, e.g., the methods invoked by an object variable of a class. Finally, the types of API elements that can satisfy the constraints at most are determined based on the pre-built KB.

Table~\ref{tab:constraint-methods-review} presents a list of constraint-based methods for Java. SnR achieves state-of-the-art performance according to the evaluations reported in \cite{DBLP:conf/icse/DongGTS22, DBLP:conf/kbse/SaifullahAR19-coster}. %~\cite{DBLP:conf/icse/DongGTS22}. %as {\color{blue}it utilizes more comprehensive constraints and makes use of refined knowledge to handle generic types.} 
SnR pre-builds a KB from a set of Jar files by extracting the classes and interfaces, their included methods and fields, and the inheritance and implementation relationships between them. For an input code snippet, SnR first attempts to repair it to a syntactically valid compilation unit using a template-based method, such that an Abstract Syntax Tree (AST) can be generated for the unit. After that, SnR extracts type constraints from the AST and represents the constraints using a declarative logic programming language, Datalog~\cite{DBLP:journals/pacmpl/MadsenL20-datalog}. Based on the pre-built KB and extracted constraints, several heuristic rules are used for type inference, e.g., minimizing the number of unique libraries used in the code snippet.

\begin{figure}%[htbp]
    \centering
    \includegraphics[width=0.9\linewidth]{figure/fig2_syntax_incorrectness.pdf}
    \caption{Example code snippet with syntax errors from the SO post `1318732'. A serious syntax error is that the constructor name, \emph{CountryFilterView}, is not the same as the class name, \emph{MyView}.}
    \label{fig:syntax-incorrectness}
\end{figure}

\begin{table}
    \centering
    \caption{Type inference results produced by two state-of-the-art methods, i.e., SnR and MLMTyper, for the code snippet shown in Fig.~\ref{fig:syntax-incorrectness}. To distinguish multiple API elements with the same name in the code snippet, two indices (i.e., the line number and the order of occurrence) are used to locate a specific API element, e.g., `VerticalSplitPanel$[\underline{3},\underline{2}]$' indicates the \underline{2nd} class `VerticalSplitPanel' at \underline{line 3}.}
    \label{tab:snr-syntax-incorrectness}
        \resizebox{\textwidth}{!}
        {
            \begin{tabular}{l|c|l|c|l} 
                \toprule
                \multicolumn{1}{c|}{\textbf{API}} & \multicolumn{2}{c|}{\textbf{\textbf{SnR}}}                       & \multicolumn{2}{c}{\textbf{MLMTyper}}                                      \\ 
                \hline
                Composite[1,1]                    & \textit{com.google.gwt.user.client.ui.Composite} & $\usym{2714}$ & \textit{android.widget.Composite}                         & $\usym{2717}$  \\
                VerticalSplitPanel[3,1]           & -                                                &               & \textit{com.google.gwt.user.client.ui.VerticalSplitPanel} & $\usym{2714}$  \\
                VerticalSplitPanel[3,2]           & -                                                &               & \textit{com.google.gwt.user.client.ui.VerticalSplitPanel} & $\usym{2714}$  \\
                HTML[9,1]                         & -                                                &               & \textit{com.google.gwt.user.client.ui.HTML}               & $\usym{2714}$  \\
                HTML[10,1]                        & -                                                &               & \textit{com.google.gwt.user.client.ui.HTML}               & $\usym{2714}$  \\
                \bottomrule
                \end{tabular}
        }
\end{table}

A major limitation of constraint-based methods is that they require the valid compilation of the input code snippet in order to extract constraints for type inference. Although some methods, e.g., SnR, address this problem using a template-based syntax repair method, there still exist a large portion of code snippets that cannot be repaired or can only be partially repaired, which obstructs the application of constraint-based methods. For example, the code snippets in SO posts often contain a lot of syntax errors. The syntax repair method used by SnR only focuses on the compilation errors that account for 38\% of the total errors in the analyzed code snippets from SO posts~\cite{DBLP:conf/issta/TerragniLC16-csnippex}
% Only 3.89\% of the SO code snippets analyzed in \cite{DBLP:conf/msr/YangHL16} could be successfully parsed by Eclipse JDT1.7's ASTParser, and only 1.00\% could be compiled.
Fig.~\ref{fig:syntax-incorrectness} shows an example code snippet from the SO post `1318732'. Table~\ref{tab:snr-syntax-incorrectness} presents the type inference results produced by SnR. As can be seen, SnR only infers the type of the class \emph{Composite}[1,1] (the two indices in `[]' are used to locate the class in the code snippet, as explained in the caption of the table) outside the definition of the class \emph{MyView} and fails to infer the types of the remaining classes. This issue is caused by the syntax error that the constructor name, \emph{CountryFilterView}, is different from the class name.

Apart from the limitation regarding code snippet compilation, constraint-based methods are also limited by 1) the coverage of the pre-built KB; 2) the richness of the type constraints included in the code snippet; and 3) the capability of the methods in extracting the constraints. Specifically, the types of API elements outside the KB cannot be inferred. For a code snippet, if an API element has multiple candidate types in the KB, in order to determine the type of the element, the code snippet should contain sufficient constraints for filtering the other candidates, and meanwhile the methods should be able to extract the constraints and use them for type inference effectively.

\subsubsection{Statistically-based Type Inference Methods.} A statistically-based method builds a statistical model from an extensive code corpus using machine learning (e.g., deep learning) techniques. The types of API elements in the code corpus are given. Using the model, the method infers the types of API elements in a code snippet by maximizing the likelihood of the code snippet. Statistically-based methods eliminate the code snippet compilation limitation by treating code snippets as plain text.

\begin{figure}
    \centering
    \includegraphics[width=0.9\linewidth]{figure/fig3_statistical_disadvantage.pdf}
    \caption{Example code snippet from the SO post `8746084'.}
    \label{fig:ase-disadvantage}
\end{figure}

\begin{table}
    \centering
        \caption{Statistically-based type inference methods.}
        \label{tab:statistical-based-review}
        \resizebox{\textwidth}{!}
        {
            \begin{tabular}{l|c|l} 
                \hline
                \multicolumn{1}{c|}{\textbf{Method}} & \textbf{Publication} & \multicolumn{1}{c}{\textbf{Summary}}                                                                                                                                                                                                                                                                   \\ 
                \hline
                STATTYPE~\cite{DBLP:conf/icse/PhanNTTNN18-statype}                             & ICSE 2018            & \begin{tabular}[c]{@{}l@{}}Based on the assumption that APIs have co-occurring regularities which can be learned\\by statistical models, STATTYPE treats the type inference task as a statistical machine \\translation~task and considers both the type context and resolution context.\end{tabular}  \\ 
                \hline
                COSTER~\cite{DBLP:conf/kbse/SaifullahAR19-coster}                               & ASE 2019             & \begin{tabular}[c]{@{}l@{}}COSTER utilizes both the local and global contexts of an API. It calculates a likelihood score, \\a~context similarity score, and a name similarity score based on a pre-built occurrence \\likelihood~dictionary to map an API element to its type.\end{tabular}           \\ 
                \hline
                RESICO~\cite{DBLP:journals/scp/VelazquezRodriguezNR23-resico}                               & SCP 2023             & \begin{tabular}[c]{@{}l@{}}RESICO uses the Word2Vec model to vectorize the API reference and its context, which \\is then fed into a machine learning classifier to obtain type recommendations.\end{tabular}                                                                                          \\ 
                \hline
                MLMTyper~\cite{DBLP:conf/kbse/HuangYXX0022-prompt}                             & ASE 2022             & \begin{tabular}[c]{@{}l@{}}MLM transforms the type inference task into a fill-in-blank task based on a prompt-tuned \\masked language model.\end{tabular}                                                                                                                                              \\
                \hline
                \end{tabular}
        }
\end{table}

\begin{table}%[htbp]
    \centering
    \caption{Type inference results produced by two state-of-the-art methods, i.e., SnR and MLMTyper, for the code snippet shown in Fig.~\ref{fig:ase-disadvantage}. Similar to Table~\ref{tab:snr-syntax-incorrectness}, two indices (i.e., the line number and the order of occurrence) are used to locate a specific API element in the code snippet, e.g., `DateTime$[\underline{2},\underline{1}]$'.}
    \label{tab:MLM-disadvantage-example}
    \resizebox{\textwidth}{!}{
        \begin{tabular}{l|c|l|c|l} 
            \toprule
            \multicolumn{1}{c|}{\textbf{API}} & \multicolumn{2}{c|}{\textbf{SnR}}                               & \multicolumn{2}{c}{\textbf{MLMTyper}}                 \\ 
            \hline
            DateTimeFormatter[1,1]            & \textit{org.joda.time.format.DateTimeFormatter} & $\usym{2714}$ & \textit{java.text.DateTimeFormatter} & $\usym{2717}$  \\
            DateTimeFormat[1,1]               & \textit{org.joda.time.format.DateTimeFormat}    & $\usym{2714}$ & \textit{java.text.DateTimeFormat}    & $\usym{2717}$  \\
            DateTime[2,1]                     & \textit{org.joda.time.DateTime}                 & $\usym{2714}$ & \textit{org.joda.time.DateTime}      & $\usym{2714}$  \\
            LocalDate[3,1]                    & \textit{org.joda.time.LocalDate}                & $\usym{2714}$ & \textit{java.time.LocalDate}         & $\usym{2717}$  \\
            \bottomrule
            \end{tabular}
    }
\end{table}

Table~\ref{tab:statistical-based-review} presents a list of statistically-based methods for Java. According to the evaluations reported in \cite{DBLP:conf/kbse/HuangYXX0022-prompt,DBLP:journals/scp/VelazquezRodriguezNR23-resico}, the prompt-tuned masked language model (MLM)-based method proposed by Huang et al.~\cite{DBLP:conf/kbse/HuangYXX0022-prompt}, referred to as MLMTyper in this work, achieves state-of-the-art performance. MLMTyper transforms the type inference task into a cloze-filling problem and uses a prompt-tuned MLM to complete the missing types of API elements. MLMTyper achieves a relatively high recall of 91\%, which is better than that (i.e., 87.5\%) of SnR~\cite{DBLP:conf/kbse/HuangYXX0022-prompt}. The improvement is mainly because MLMTyper overcomes the compilation limitation and would not fail to give inference in any cases.

A major limitation of statistically-based methods is that they rarely take the syntax knowledge of APIs and the type constraints in code snippets into consideration, which may lead to low precision in some cases. This limitation becomes more obvious when facing APIs or contexts that are less popular in the training code corpus \cite{DBLP:conf/kbse/HuangYXX0022-prompt, DBLP:conf/kbse/SaifullahAR19-coster}. Fig.~\ref{fig:ase-disadvantage} shows a code snippet from the SO post `8746084'. Table~\ref{tab:MLM-disadvantage-example} presents the top-1 types of the classes inferred by MLMTyper. 
MLMTyper correctly predicts \emph{DateTime}[2,1] as \emph{org.joda.time.DateTime} but mistakenly predicts the types of the other three classes. For example, the return type of the method \emph{org.joda.time.DateTime.toLocalDate()} is \emph{org.joda.time.LocalDate}. However, MLMTyper does not consider the syntax knowledge and thus predicts the wrong type for \emph{LocalDate}[3,1].

\subsubsection{Insight.}
As explained above, both constraint-based type inference methods and syntactically-based type inference methods have their own limitations. Constraint-based methods often have a relatively high precision by leveraging the syntax knowledge of APIs and the constraints in code snippets, however their recall may be low due to several factors, e.g., the compilation failure of code snippets and the low coverage of the pre-built KB. In contrast, statistically-based methods do not require to compile code snippets and can infer candidate types for all API elements, which may improve the recall. However, the precision of the methods may be low since they do not consider the constraints in code snippets and thus lead to wrong types. Tables~\ref{tab:snr-syntax-incorrectness} and~\ref{tab:MLM-disadvantage-example} present the type inference results produced by SnR and MLMTyper for two code snippets. SnR achieves a high precision of 100\% on both cases but a low recall of 20\% on the first case. Compared with SnR, MLMTyper achieves a higher recall of 80\% and also a lower precision of 80\% on the first case. On the second case, both precision and recall of MLMTyper are lower than those of SnR.

\textbf{We further observe from the table results that the type inference results produced by SnR and MLMTyper exhibit a certain degree of complementarity.} As an example, for the code snippet shown in Fig.~\ref{fig:syntax-incorrectness}, SnR correctly infers the type of the class \emph{Composite}[1,1] but fails to infer the types of the other classes, while MLMTyper predicts wrong type for \emph{Composite}[1,1] but correct types for the others. Based on this observation, better performance could be achieved by integrating constraint-based and statistically-based methods. Following this insight, we propose an integrated type inference framework, which is elaborated in the following section.

